Unsatisfied Today, Satisfied Tomorrow: a simulation framework for performance evaluation of crowdsourcing-based network monitoring

Network operators need to continuosly upgrade their infrastructures in order to keep their customer satisfaction levels high. Crowdsourcing-based approaches are generally adopted, where customers are directly asked to answer surveys about their user experience. Since the number of collaborative users is generally low, network operators rely on Machine Learning models to predict the satisfaction levels/QoE of the users rather than directly measuring it through surveys. Finally, combining the true/predicted user satisfaction levels with information on each user mobility (e.g, which network sites each user has visited and for how long), an operator may reveal critical areas in the networks and drive/prioritize investments properly. In this work, we propose an empirical framework tailored to assess the quality of the detection of under-performing cells starting from subjective user experience grades. The framework allows to simulate diverse networking scenarios, where a network characterized by a small set of under-performing cells is visited by heterogeneous users moving through it according to realistic mobility models. The framework simulates both the processes of satisfaction surveys delivery and users satisfaction prediction, considering different delivery strategies and evaluating prediction algorithms characterized by different prediction performance. We use the simulation framework to test empirically the performance of under-performing sites detection in general scenarios characterized by different users density and mobility models to obtain insights which are generalizable and that provide interesting guidelines for network operators.

==> simframework.tex <==
\section{Simulation Framework} \label{sec:framework}
In order to answer to questions \ref{Q1}-\ref{Q5}, we propose a simulation framework composed of several building blocks, illustrated in Figure \ref{fig:simframe}. The following sections provide details on each component of the framework.

	\subsection{Topology Generator (TG)} The TG is responsible of generating mobile network instances composed of a set of network sites $\mathcal{J}, |\mathcal{J}|=J$, deployed in a realistic scenario (e.g., urban or rural). The TG also defines which sites $\mathcal{J}_\text{u} \subset \mathcal{J}, |\mathcal{J}_\text{u}|=\Omega<J$, are malfunctioning or under-performing in a particular network topology. The selection is performed according to a random process, specified in input. In this work we consider a uniform distribution (i.e., all network sites have the same probability of being set as under-performing), although an operator may use any other distribution. As an example, sites characterized by a higher level of congestion (e.g., visited by high number of users) may be selected as under-performing with a higher probability. Both the total number of sites $J$ and the number of malfunctioning sites $\Omega$ are user-specific and therefore represent hyper-parameters of the simulation framework.
	
	% %\subsection{Topology Generator}\label{sec:upsites}
	% %AP: per ora questo sblocco sfrutta i tempi di visita, ma nella figura non c'è la freccia in input dal simulatore di mobilità.
	% The Topology Generator (TG) models the presence in the network of a group of under-performing sites, which may determine negative service experiences to the visiting users. To do this, it defines a discrete probability distribution $P_c^{\mathcal{J}}$ over the set $\mathcal{J}$ of network sites, such that most \textit{congested} sites (i.e., most visited sites) have higher probability to show problems in operational conditions, thus being under-performed or malfunctioning.
	% %Generally speaking, when a network site is required to provide its visitors with an amount of resources that exceed the available resource budget (e.g., in case of heavy traffic loads or high number of connections) then the overall experience of the visitors could be negative.
	% This allows us to write the probability $p_c(j)$ that site $j$ is an anomaly as it follows:
	% \begin{align}
	%  &\quad& p_{c}(j)= \frac{\sum\limits_{i \in I} {t\textsubscript{i,j}}}{\sum\limits_{i \in I, j \in J} {t\textsubscript{i,j}}} \hspace{5mm}, &\quad&\forall{j} \in \mathcal{J}
	% \end{align}
	% where $t\textsubscript{i,j}$ is the time that user $i$ has spent in network site $j$. Then, for each network site $j$, the TG proceeds with one of the two following operations:
	% \begin{enumerate}
	%     \item with probability $P_{cong}$, the anomaly is due to traffic congestion and site $j$ is marked as anomalous with probability $p_c(j)$,
	%     \item with probability $1 - P_{cong}$, the anomaly is due to unknown reasons and site $j$ is marked as anomalous with probability $0.5$, i.e., randomly.
	% \end{enumerate}
	% Note that $P_{cong}$ is a hyper-parameter of the framework and can be arbitrarily tuned to simulate the desired scenario. The selection process is repeated for each $j$ $\in$ $\mathcal{J}$ and finally produces the set $\mathcal{J}_u$ of under-performing network sites. For the sake of clarity, we underline that $\mathcal{J}_u$ is a subset of the overall set of sites $\mathcal{J}$. The size $\omega$ of $\mathcal{J}_u$ (expressed as a fraction of the size of set $\mathcal{J}$) is defined \textit{a priori} and therefore represents a hyper-parameter of the framework.

	\subsection{User Mobility Manager (UMM)}
	The UMM models the mobility of the population users $\mathcal{U}$ through the cellular network simulated by the TG. In particular, the UMM leverages a human mobility model which defines for the $i$-th user i) which network cells/sites are visited and ii) for how long. Several models are available in the literature to simulate the statistical properties of human mobility in urban or rural areas\cite{hyytia2007random, lee2009slaw, munjal2011smooth, song2010modelling}. In this work we consider the model proposed in \cite{song2010modelling}, which is based on the following observations: i) humans have a periodic tendency to return to previously visited places, ii) humans spend most of their time in a few number of locations and iii) the distributions of the time spent by a user in a loaction $\Delta t$ and the distance covered between two sightings $\Delta r$ are fat-tailed, i.e. $P(\Delta r) \sim |\Delta r|^{-1-\alpha}$ and $P(\Delta t) \sim |\Delta t|^{-1-\beta}$.
	 %These observations make human trajectories substantially different from random walk-based models \cite{gonzalez2008understanding}.
	In details, the mobility model implemented in the UMM works according to different steps, as illustrated in Figure \ref{fig:mobilityalgorithm}:
	\begin{itemize}
		\item \textit{Initialization:} let $S_i$ be an integer variable which counts the number of distinct locations visited by the $i$-th user, initially set to 1. At startup, each user is associated to one site in the network topology, chosen at random.  Then, each user waits for a period of time $\Delta t$ and eventually decides whether to explore a new location (Exploration step) or to return to an already visited site, including the current one (Preferential return step).
		\item \textit{Exploration:} with probability $P_{new} = \rho S_i{^{-\gamma}}$, the user jumps in a random direction $\theta$, uniformly distributed in the range $[0, 2\pi)$ and with a jump length of $\Delta r$. The closest site to the landing location will be visited by the user. As the user moves to this new position, the number of previously visited locations increases from $S_i$ to $S_i + 1$.
		\item \textit{Preferential Return:} with probability $1-P_{ret}$, the user returns to a previously visited location with a probability proportional to the number of visits the user previously had to that location. 
	\end{itemize}
	These steps are repeated independently for each user: at each iteration the UMM updates the vector $\textbf{t}_i \in \mathbb{R}_{\ge 0}^J$ whose entries $t_{i,j}$ corresponds to the visit times of the $i$-th user in the $j$-th network site. The process ends when the total visit time for each user is equal to the simulation time horizon $T$, i.e., when $\sum_j{t_{i,j}} = T, \,\,\forall i$. The parameters controlling the user's tendency of exploring a new place $\rho$ and $\gamma$, as well as the fat-tail distribution parameters for the jump sizes $\alpha$ and the waiting times $\beta$ can be modified according to the specific case under consideration. We detail the choice of such hyper-parameters in Section \ref{sec:experiment}.
	
	\begin{figure}[t]
	    \centering
	    \includegraphics[scale=0.5]{pics/mobility_alg_v2.png}
	    \caption{Considering a generic user $i$, S equals the cardinality of the set of visited places, circles stems for the sites already visited by the user while their size represents the probability that the user visits the corresponding network site.}
	    \label{fig:mobilityalgorithm}
	\end{figure}
	
	% This leads to two main mechanisms for characterizing users mobility in a cellular network, namely \textit{Exploration} and \textit{Preferential Return}.

% 	To show how these two mechanisms work, we depict in Figure \ref{fig:mobilityalgorithm} the evolution of a user's trajectory in the network. In this example, a user has visited $S=4$ distinct network sites (the four coloured circles on the lest side of the Figure) and he/she is currently visiting one of them. Note that the area of a circle is proportional to the number of times the user has visited the corresponding location, i.e., to the probability that the user visits that location. Assuming the user to be leaving the currently visited network site, he/she has two possibilities:
% 	\begin{itemize}
% 	    \item Exploration: to explore a new, unknown location. This happens with probability $P_{new} = \rho S^{-\gamma}$, where $\rho$ is a scaling factor and $\gamma$ is an hyper-parameter that controls the individual's tendency of exploring a new place versus returning to a previously visited one.
% 	    \item Preferential Return: to return to a previously visited location. This happens with probability $P_{ret} = 1- \rho S^{-\gamma}$. The choice of the location to which to return is done according to a probability distribution defined over the set of already visited places.
% 	\end{itemize}
% 	Note that UMS processes each user independently from the others, meaning that their trajectories can be computed in parallel for all the users for each time step. Considering a given user, at time $t=0$ he/she is assigned with a starting location, corresponding to the GPS coordinates of the starting network site. The starting location is drawn from a probability distribution which takes into account the residential densities of the different areas in the city, such that network sites located in highly residential areas are more likely chosen as starting sites. Then, the user waits for a time equal to $\Delta$t $\in$ $P_{WT}$ and eventually decides whether to explore a new location (thus moving to the next network site) or to return to an already visited site (including the possibility of remaining in the currently visited one). The process repeats for each next location, until the sum of the user's waiting times in each visited site saturates the observation period. When exploring, the user jumps in a random direction $\theta$, where $\theta$ is uniformly distributed in the range $[0, 2 \cdot \pi)$ [rad] while the jump length $\Delta$r is drawn from $P_{HD}$.
	
	% Note that the UMG processes each user independently from the others, meaning that users trajectories can be computed in parallel at each time step. At the end of the process, the UMG returns for each user $i$ a vector $\textbf{t}$(i) whose entries are the times $t\textsubscript{i,j}$ spent by the $i-th$ user in each network site $j$. For further details about the model, refer to \cite{song2010modelling}. According to the value of the parameter $\gamma$, we define two mobility scenarios:
% 	\begin{itemize}
% 	    \item \textbf{Theoretical Model} (TM): it reproduces the hyper-parameters setup described in \cite{song2010modelling}, where a data-driven approach is used to statistically estimate the values of the hyper-parameters. In particular, $\gamma$ is set equal to $0.21$;
% 	    \item \textbf{Empirical Model} (EM): it reproduces the users mobility pattern observed from real empirical data regarding the mobility of $1500$ customers throughout a city-wide LTE network of a big European cellular operator. In this case, the value of $\gamma$ is set equal to $3$.
% 	\end{itemize}
% 	We will discuss later in Section \ref{sec:experiment} about the characteristics of both the considered scenarios.
	
	
	\subsection{User Profiler (UP)} 
	As illustrated in Figure \ref{fig:simframe}, the UP leverages the network topology created by the TG and the mobility information output by the UMM to simulate the users (subjective) reactions $\mathbf{s}$ to the corresponding experiences in the network. In this work we assume that $\mathbf{s} \in [0,1]^I$, i.e., each user is either satisfied or dissatisfied with the network service (TODO: aggiungere una frase con un paio di lavori che trattano la soddisfazione in maniera binaria). In details the $i$-th user reaction $s_i$ is defined as:
    \begin{equation}
       s_i=
       \begin{cases}
         1, & \text{if $i$-th user is dissatisfied with her network service}\\
         0, & \text{otherwise}.
       \end{cases}
     \end{equation}
	 
It is well known from the literature that the duration of a network disservice has great impact on the experience perceived by a user. As an example, in the case of video streaming, QoE is primarily influenced by the frequency and duration of stalling events \cite{hossfeld2011quantification, nam2016qoe}. Similarly, for web browsing, the number and duration of IRAT handovers is shown to have a strong negative impact on user experience \cite{balachandran2014modeling}. In both cases users are observed to tolerate a certain amount of disservice before expressing a negative opinion: for video streaming, one stalling event per clip is acceptable as long as its duration is below 3 seconds, while for web browsing a single IRAT handover is generally tolerated.
	
Following these observations, it is reasonable to link the user satisfaction $s_i$ to the time spent in under-performing or malfunctioning network sites. Operatively, the UP leverages the set of under-performing sites $\mathcal{J}_u$ and the user visit times $t_{i,j}$ to generate user satisfaction according to the following:
    \begin{equation}
       s_i=
       \begin{cases}
         1, & \text{if}\,\, \sum_{j \in \mathcal{J}_c} t_{i,j} \geq u_i T\\
         0, & \text{otherwise}.
       \end{cases}
     \end{equation}
%\subsection{User Profiler}\label{sec:UT}
 %$\in$ $\mathcal{R}$
%The User Profiler (UP) simulates the subjective reactions of cellular users to their experience in the network. Let $s(i) \in \textbf{s}$ be a binary satisfaction label representing the reaction of user $i$, which equals $1$ if the user is \textit{dissatisfied} about his/her experience in the network, while it equals $0$ otherwise. 

%Considering the set of under-performing sites $\mathcal{J}_u$ (which is an input to this block as shown in Figure \ref{fig:simframe}), the UP sets $s(i)=1$ for all users $i$ that satisfy the following condition: 
%\begin{align}\label{eq:user_sat}
%   &\quad& \sum_{j \in \mathcal{J}_c} t\textsubscript{i,j} \geq u_i * \mathcal{H} &\quad&\forall{j} \in \mathcal{J}
%\end{align}
where $T$ is the simulation time horizon and $u_i$ is a percentage value corresponding to the \textit{user tolerance}. In other words, we assume that each user has a specific patience level with respect to negative network experiences. Intuitively, the higher the tolerance of a user the more she will tolerate low service quality during her network activity. To model the heterogeneity of the users, we assume that the user tolerance $u_i$ is a Gaussian-distributed random variable with mean $\mu$ and standard deviation $\sigma$, i.e., $u_i \sim \mathcal{N}(\mu, \sigma^2)$. Later in Section \ref{sec:sensan} we will discuss about the choice of their values.




%Therefore, $s(i)=1$ if the cumulative relative time spent by user $i$ in each visited under-performing site (if any) is greater than a user dependent time activation threshold, which is referred to as \textit{user tolerance} ($u_i \in [0,1]$). The rationale behind this rule is that if a user spends most of his/her time in an under-performing site (or equivalently in a group of them), then he/she will report a negative feedback to the operator. In other words, we assume that each user has a unique patience level (i.e., $u_i$) with respect to negative network experiences. Intuitively, the higher the tolerance of a user the more he/she will tolerate low service quality during his/her network activity. 

%Considering that the population of users is heterogeneous, we decided to draw for each user $i$ the corresponding tolerance value from a Gaussian-distributed random variable $\mathcal{N}$ with mean $\mu$ and standard deviation $\sigma$, i.e., $u_i \sim \mathcal{N}(\mu, \sigma^2)$. Later in Section \ref{sec:sensan} we will discuss about the choice of their values.\par
Finally, we observe that the reported user satisfaction depends also on factors completely unrelated with the network service itself, such as the ones relative to users personal attitudes and expectations~\cite{boz2019mobile}. The UP models such noisy behaviours by generating a percentage $\psi$ of the satisfaction labels $s_i$ at random, regardless of the sites visited by users and their tolerance. Again, $\psi$ represents a hyper-parameter of the model that can be set by the operator to simulate different population types.	
	
	\subsection{Survey Delivery (SD)} 
	Any crowdsourcing-based network monitoring system is limited by the associated \textit{network coverage}, i.e., the percentage of sites visited by users answering the surveys, as it is not possible to detect under-performing sites for which no information from users is available.
	As aforementioned, the number of users which answer to surveys is generally small compared to the total number of customers, and the set of corresponding \textit{Ground Truth} responses $\mathbf{s}\textsubscript{gt}$ is much smaller than $\mathbf{s}$. The SD component of the proposed framework simulates the process of administrating satisfaction surveys to the customers, and can therefore be tought of as a sampling process of the true user reactions.
In this paper we consider two scenarios for the surveys delivery strategy:
	
	
	
	%The output $\mathbf{s}\textsubscript{gt}$ of this block corresponds to the \textit{Ground Truth} (GT) knowledge base available to the operator to proceed with the under-performing sites ranking/detection task. As discussed in Section X, since usually users responses are much less than the overall number of issued surveys, the set of responses $\mathbf{s}\textsubscript{gt}$ is much smaller than $\mathbf{s}$, i.e., the Survey Delivery process acts as a \textit{sampler} of user reactions.

%The Survey Delivery (SD) block is in charge of simulating the process of administration of satisfaction surveys from a cellular operator to its customers. The higher the \textit{response rate} ($\eta$) of a surveying campaign (i.e., the percentage of users answering the surveys with respect to the overall number of delivered surveys) the better is the statistic representation of the users population. We will consider two different surveys delivery strategies:
\begin{itemize}
		\item Random Delivery (RD): in the most general case, we assume that the set of users answering the surveys is randomly sampled from the total population. This strategy is represented in Figure \ref{fig:random}, where user icons represent those users who replied to the received survey. In this (unlucky) example the operator has low network coverage, as the received responses do not cover under-performing sites in the network.
		\item Optimized Delivery (OD): with this policy, depicted in Figure \ref{fig:optimum}, the operator delivers surveys in a way to maximize the network coverage. This is done by leveraging the user-visit times $t_{i,j}$ to set up an optimization problem (formalized in XXX) that selects the best set of users whose responses would allow to maximize the network coverage. Clearly, In this case, we assume that the operator puts in place incentives in the voting procedure, such that a selected user is rewarded for its answer (e.g. with premium data plan access for limited time or other incentives).			
		%From now on, we will assume that a network site is covered if it has been visited at least by $n$ replying users, each one visiting the site for at least $l\%$ of the observation period. This scenario is depicted in Figure \ref{fig:optimum}, where replying users are distributed in the network such that the majority of the sites are covered. Intuitively, this lets the operator have a more clear understanding about network users satisfaction. Note that the greater the values of $n$ and $l$ the stricter the definition of network coverage, as either more or longer visiting users are needed to cover a network site. Both $n$ and $l$ represent system hyper-parameters that can be chosen a priori for modelling purposes.
\end{itemize}
\begin{figure}[t]
\centering     
\subfigure[RD: low network coverage \newline scenario]{\label{fig:random}\includegraphics[width=0.38\textwidth]{pics/GTusersRandom.png}}
\subfigure[OD: high network coverage \newline scenario]{\label{fig:optimum}\includegraphics[width=0.4\textwidth]{pics/GTusersOpt.png}}
\caption{Strategies for the delivery of satisfaction surveys: a network coverage perspective. User icons refer to the users who replied to the received surveys, while blackish and redish base stations refer to regular and anomalous network sites respectively.}
\label{fig:deliveries}
\end{figure}
From a simulative perspective, the SD block samples the set of users reactions $\mathbf{s}$ and returns a set of GT users feedbacks $\mathbf{s}\textsubscript{gt}$.
%Figure \ref{fig:simframe} depicts the architecture of a framework that an operator can leverage to simulate the application of the detection process to different network scenarios. On the left side of the figure, we represent the \textit{generation} of the network instance and data that will be considered by the detection system to recognize under-performing network sites. First, a cellular network instance is generated by the \textit{Topology Generator}, such that some of the network sites are assumed to be under-performing sites (in Figure \ref{fig:simframe}, those belonging to the set $\mathcal{J}_u$). Secondly, we simulate the visit of the network for a given observation period by a group of cellular users, which moves according to a mobility model set by the \textit{User Mobility Generator}. For each user in the population, such block defines i) which network sites are visited and ii) for how long.
%Leveraging the information about the location of under-performing sites in the network and the users per-site visit times, the \textit{User Profiler} can then simulate the users (subjective) reactions $\mathbf{s}$ to the corresponding experiences in the network. Finally, the \textit{Surveys Delivery} block simulates the administration of satisfaction surveys to the considered users. The output $\mathbf{s}\textsubscript{gt}$ of such block corresponds to the \textit{Ground Truth} (GT) knowledge base available to the operator to proceed with the detection task. As discussed in the previous Section, since usually users responses are much less than the overall number of issued surveys, the set of responses $\mathbf{s}\textsubscript{gt}$ is a subset of $\mathbf{s}$, i.e., the Survey Delivery process acts as a \textit{sampler} of users reactions.\par

%At this point, the detection system introduced in the previous Section (which corresponds to the core of the framework represented in Figure \ref{fig:simframe}) can be used to detect under-performing sites in the network. The system will leverage: i) the user-specific cell visit times information generated by the UMM; ii) the set of GT survey responses generated by the SD block, available only for a subset of the population; iii) a pre-trained ML model $f(\cdot)$, to predict the satisfaction feedback of all those users who did not answer a survey (i.e., non-GT users). Note that the ML model is assumed to be already trained and we are not interested in detailing which learning features belong to $\mathbf{X}_\text{a}$ and $\mathbf{X}_\text{na}$. Finally, the system provides the operator with a ranked set $\hat{\mathcal{J}}_\text{u}$ of predicted under-performing sites, that is eventually compared with the set $\mathcal{J}_\text{u}$ to assess the detection performance. In the following Sections we describe in details the operations performed by the different blocks of the framework. 
%The aim of the system is to leverage both users side objective information (e.g., which network sites the users have visited and for how long) and subjective satisfaction feedbacks to recognise and detect anomalies in the network. In order to evaluate the performance of the detection system, we implement a realistic simulation framework where an heterogeneous group visits the network and expresses a feedback regarding the quality of the experienced cellular service. 
%Assuming that some network sites are under-performing (and thus \textit{anomalous}), some of the users visiting those sites will provide the operators with negative satisfaction feedbacks, which will be leveraged by the system to detect the location of the anomalies. The simulation framework is added to the back-end of the detection system to provide it with (realistic) simulative network data. 
%In particular, the simulation framework is composed of four parts: the User Mobility Simulator (UMS), which simulates the mobility of a group of users in a cellular network, ii) the Anomalies Generator (AG), which simulates the presence of the anomalies that have to be detected by the system, iii) the User Profiler (UP), which simulates users' reaction to bad quality network events and the Performance Evaluator (PE), which evaluates the detection accuracy $A$ of the system. Note that the simulation framework is characterized by a group of hyper-parameters that can be flexibly tuned by the operator to simulate a large variety of network scenarios: details will be given in the following Sections. To conclude, we show in Figure \ref{fig:simframe} the complete architecture where the detection system is integrated into the simulation framework.
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/new_system_diagram_2.pdf}
    \caption{Architecture of a simulation framework to test the anomaly detection system.}
    \label{fig:simframe}
\end{figure}
%The proposed framework will be applied to recognize the presence of (simulated) anomalies in the LTE network of a big European cellular operator, currently operative in a mid-size European city. The considered network, which is shown in Figure \ref{fig:voronoi}, comprises of $136$ network sites. 
%\begin{figure}[t]
%    \centering
%    \includegraphics[scale=0.5]{pics/voronoi_v2}
%    \caption{Voronoi representation of the considered LTE network.}
%    \label{fig:voronoi}
%\end{figure}

%We will simulate the visitation of the network by an heterogeneous group of users who eventually will express a feedback regarding the experienced cellular service. Moreover, we will assume that some LTE sites are under-performing, and thus \textit{anomalous}. For this reason, some of users visiting anomalous sites will provide the operators with negative satisfaction feedbacks. Note that different users may perceive differently the quality of a network event, thus for same observed network performance different users may give different feedbacks. The aim of the framework is to leverage both objective information (e.g., which network sites the users have visited and for how long) and users' subjective QoE evaluation to recognise and detect the anomalous sites in the network. 
%	\item \textbf{Data Generation Blocks}: these blocks generate the data that will be used to simulate the anomaly detection task. In this group, we can recognize: i) the User Mobility Block (UMB), which simulates the mobility of a group of users in a cellular network, ii) the Anomalies Generator Block (AGB), which defines the location of the anomalies in the cellular network that have to be detected and iii) the User Profile Block (UPB), which simulates users' reaction to bad quality network events;
%	\item \textbf{Operative Blocks}: these blocks leverage the data at the output of the Data Generation Blocks and simulate the anomaly detection process. In particular, we distinguish: i) the Quality of Experience Block (QEB), which exactly measures the QoE of a subset of the visiting users while \textit{predicts} that one of the remaining users and the Anomaly Detection Block (ADB), which performs the detection of the anomalies in the network. Note that the same operations performed by QEB and ADB can be done leveraging \textit{real} data similar to those generated by the Data Generation Blocks.
%\end{enumerate}
%The output of the framework is the anomaly detection error, computed by the Detection Error Block (DEB). In the following sections, we will discuss in details about the implementation of both Data Generation and Operative Blocks.
%\begin{figure}[t]
%    \centering
%    \includegraphics[scale=0.5]{pics/framework_architecture}
%    \caption{Architecture of the proposed anomaly detection framework.}
%    \label{fig:framework}
%\end{figure}
%Referring to Figure \ref{fig:framework}, which depicts the architecture of our anomaly detection framework, we can group the building blocks as it follows:
%\begin{enumerate}

% %-----------Mobility model-----------
% \subsection{User Mobility Generator}\label{sec:mobilitymodel}
% The User Mobility Generator (UMG) models the mobility of a population of users throughout a given cellular network. In literature, authors have proposed several models \cite{hyytia2007random, lee2009slaw, munjal2011smooth, song2010modelling} to embed the statistical properties of human mobility traces and simulate their evolution in urban areas. In this work we consider the model proposed by \cite{song2010modelling}, which is based on the following observations: i) humans have a periodic tendency to return to previously visited places and ii) humans spend most of their time in a few number of locations, this making human trajectories substantially different than random walk-based models \cite{gonzalez2008understanding}. These observations let the authors in \cite{song2010modelling} recognize two principle mechanisms that characterize users mobility in a cellular network,  namely \textit{Exploration} and \textit{Preferential Return}.
% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.5]{pics/MobilityModelSchem.png}
%     \caption{Considering a generic user $i$, S equals the cardinality of the set of visited places, circles stems for the sites already visited by the user while their size represents the probability that the user visits the corresponding network site.}
%     \label{fig:mobilityalgorithm}
% \end{figure}
% To show how these two mechanisms work, we depict in Figure \ref{fig:mobilityalgorithm} the evolution of a user's trajectory in the network at a given time instant $t$. In this example, the user $i$ has visited $S=4$ distinct network sites (i.e., the four coloured circles on the lest side of the Figure) and he/she is currently visiting one of them. Note that the area of a circle is proportional to the number of times the user has visited the corresponding location, i.e., to the probability that user $i$ visits that location. Assuming the user to be leaving the currently visited network site, he/she has two possibilities:
% \begin{itemize}
%     \item Exploration: to explore a new, unknown location. This happens with probability $P_{new} = \rho S^{-\gamma}$, where $\rho$ is a scaling factor and $\gamma$ is an hyper-parameter that controls the individual's tendency of exploring a new place versus returning to a previously visited one.
%     \item Preferential Return: to return to a previously visited location. This happens with probability $P_{ret} = 1- \rho S^{-\gamma}$. The choice of the location to which to return is done according to a probability distribution defined over the set of already visited places.
% \end{itemize}
% Note that the UMG processes each user independently from the others, meaning that users trajectories can be computed in parallel at each time step. At the end of the process, the UMG returns for each user $i$ a vector $\textbf{t}$(i) whose entries are the times $t\textsubscript{i,j}$ spent by the $i-th$ user in each network site $j$. For further details about the model, refer to \cite{song2010modelling}. According to the value of the parameter $\gamma$, we define two mobility scenarios:
% \begin{itemize}
%     \item \textbf{Theoretical Model} (TM): it reproduces the hyper-parameters setup described in \cite{song2010modelling}, where a data-driven approach is used to statistically estimate the values of the hyper-parameters. In particular, $\gamma$ is set equal to $0.21$;
%     \item \textbf{Empirical Model} (EM): it reproduces the users mobility pattern observed from real empirical data regarding the mobility of $1500$ customers throughout a city-wide LTE network of a big European cellular operator. In this case, the value of $\gamma$ is set equal to $3$.
% \end{itemize}
% We will discuss later in Section \ref{sec:experiment} about the characteristics of both the considered scenarios.
 

%\par The UMS models the mobility of cellular users throughout the network and generates the \textit{mobility matrix} $\mathcal{T}$. Let us consider a set of users $\mathcal{I}$ of size $N$ that visit a set of network sites $\mathcal{J}$ of size $M$. Therefore, $\mathcal{T}$ is composed by $N$ entries $\textbf{t}(i) = [t_{i, 1}, \cdots, t_{i, M}]$, where $t_{i, j}$ equals the time spent by user $i$ in site $j$. The visit times $t_{i, j}$ are generated according to the human mobility model proposed in \cite{song2010modelling}, which describes: i) how users move from a starting location to a final one (a process statistically described by the distribution of \textit{Human Displacement} and the mechanism of \textit{Ultra-Slow Diffusion}), ii) how long users wait in a given location before moving to the next one (statistically described by the distribution of \textit{Users Waiting-Times}), iii) the mechanism behind the choice to visit a given location (for a given user, each location is associated with a \textit{Visitation Frequency}) and iv) the decreasing tendency of users to visit new and unknown locations (referred to as \textit{Users Returning-Addiction}).\\
%As a first approximation, the trajectory of a user can be explained observing that that the distributions $P_{HD}$($\Delta$r) and $P_{WT}$($\Delta$t) of respectively Human Displacement and Users Waiting-Times are fat-tailed, i.e.:
%\begin{align}
%&P_{HD}(\Delta r)\sim |\Delta r|^{-1-\alpha} \\
%&P_{WT}(\Delta t)\sim |\Delta t|^{-1-\beta}
%\end{align}
%where $\alpha$ and $\beta$ are hyper-parameters of the model and rule the exponential decay of the probability distributions. 
%%In \cite{song2010modelling}, a data-driven approach is used to statistically estimate the values of $\alpha$ and $\beta$, which in this work are set equal to their mean value, i.e., $0.55$ and $0.8$ respectively.\\
%While on the one hand fat-tailed distributions are used to describe random walk processes (such as Levy walks or Continuous-Time Random Walk (CTRW)), on the other hand it can be shown \cite{song2010modelling} that the knowledge of $P_{HD}$($\Delta$r) and $P_{WT}$($\Delta$t) is not enough to fully capture and explain the evolution of users paths in a cellular network. In particular, the following further properties need to be modelled: 
%%Similar statistic features can be observed either in the Lévy walks or in the Continuous-Time Random Walk (CTRW), that are random walk random processes. However, 
%%which are partially characterized by non-random features. 
%\begin{enumerate}[label=\Alph*]
%    \item \textit{Users Returning-Addiction}\label{ra}: it refers to the tendency of a moving object to return to an already visited location. We define $S(t)$ as the number of distinct locations $S$ visited at time $t$ by an object randomly moving in time as it follows:
%    \begin{equation}
%    S(t) \sim t^{x}
%    \end{equation}
%    where the value of $x$ depends on the statistical features of the object's walk. In the case of humans moving in a cellular network, $x$ is on average lower than 1, thus indicating a decreasing tendency of cellular users to visit new places at large time-scales; 
%    \item \textit{Visitation Frequency}\label{vf}: it refers to the frequency $v_{i,j}$ with which a user $i$ visits site $j$. It can be measured as the ratio between the number of visits of user $i$ to site $j$ and the overall number of visits of such user to all the other sites. In this work, we will consider $v_{i,j}$ as an approximation of the probability that user $i$ visits network site $j$. While such probability is expected to be asymptotically uniform for random walks, this is not the case for human traces, which are usually characterized by uneven visitation patterns;
%    \item \textit{Ultra-Slow Diffusion}\label{usd}: it refers to the drift of an object's trajectory with respect to the starting point. Due to humans tendency to return home on a daily basis, human walks are considered \textit{ultra-slow} diffusive processes.
%    %in contrast with CTRW, where the longer we observe a trajectory the further it will drift away from its initial position, in human mobility patterns there is the tendency to return home on a daily basis, this suggesting a 
%\end{enumerate}
%
%\begin{figure}[t]
%    \centering
%    \includegraphics[scale=0.5]{pics/MobilityModelSchem.png}
%    \caption{Considering a generic user $i$, S equals the cardinality of the set of visited places, circles stems for the already visited sites while their size represents the visitation frequencies $v_{i,j}$.}
%    \label{fig:3.2}
%\end{figure}
%Figure \ref{fig:3.2} depicts the algorithm implemented by the UMS to determine the evolution of a user's trajectory in the network at a given time instant $t$. In this example, the user $i$ has visited $S=4$ distinct locations (i.e., the four coloured circles on the lest side of the Figure) and he/she is currently visiting one of them. Note that the area of the coloured circles is proportional to the number of times the user has visited the corresponding locations, i.e., to the visitation frequency $v_{i,j}$. Supposing the user to be leaving the currently visited location, he/she has two possibilities:
%\begin{itemize}
%    \item \textbf{Exploration}: to explore a new, unknown location. This happens with probability $P_{new} = \rho S^{-\gamma}$, where $\rho$ is a scaling factor and $\gamma$ is an hyper-parameter that controls the individual's tendency of exploring a new place versus returning to a previously visited one. This possibility captures property \ref{ra} of human mobility patterns. 
%    \item \textbf{Preferential Return}: to return to a previously visited location. This happens with probability $P_{ret} = 1- \rho S^{-\gamma}$. The choice of the location to which to return is done according to a probability distribution defined over the set of already visited places. In particular, the probability that user $i$ will return to place \textit{j} equals $v_{i,j}$. This possibility captures properties \ref{vf} and \ref{usd} of human mobility patterns.
%\end{itemize}
%Note that UMS processes each user independently from the others, meaning that their trajectories can be computed in parallel for all the users for each time step. Considering a given user, at time $t=0$ he/she is assigned with a starting location, corresponding to the GPS coordinates of the starting network site. The starting location is drawn from a probability distribution which takes into account the residential densities of the different areas in the city, such that network sites located in highly residential areas are more likely chosen as starting sites. Then, the user waits for a time equal to $\Delta$t $\in$ $P_{WT}$ and eventually decides whether to explore a new location (thus moving to the next network site) or to return to an already visited site (including the possibility of remaining in the currently visited one). The process repeats for each next location, until the sum of the user's waiting times in each visited site saturates the observation period. When exploring, the user jumps in a random direction $\theta$, where $\theta$ is uniformly distributed in the range $[0, 2 \cdot \pi)$ [rad] while the jump length $\Delta$r is drawn from $P_{HD}$. Given the GPS coordinates of the user's Current Location $(lat_{CL}, long_{CL})$, the coordinates of his/her Next Location $(lat_{NL}, long_{NL})$  are computed as it follows:
%\begin{align}
%&lat_{NL} = \arcsin(\sin(lat_{CL})) \cdot \cos(\frac{\Delta r}{R}) + cos(lat_{CL}) \cdot \sin(\frac{\Delta r}{R}) \cdot cos(\theta)\\
%&long_{NL} = long_{CL} + \arctan2(y,x)\\
%&y = \sin(\theta) \cdot \sin(\frac{\Delta r}{R}) \cdot \cos(lat_{CL})  \\
%&x = \cos(\frac{\Delta r}{R}) - \sin(lat_{CL}) \cdot \sin(lat_{NL})
%\label{eq:coordnew}
%\end{align}
%where $R = 6372.79$ [Km] is the radius of the Earth (approximated as a sphere) and $\arctan2(y,x)$ equals the angle $\alpha$ [rad] in the Euclidean plane between the x-axis and the ray to the point of coordinates (x,y), with $x \geq 0$ and $y \neq 0$.%, as shown in Figure \ref{fig:3.4}.
%%\begin{figure}[H]
%%    \centering
%%    \includegraphics[scale=0.6]{pics/atan2.png}
%%    \caption{Graphical representation of the function arctan2(y,x).}
%%    \label{fig:3.4}
%%\end{figure}


%In this work we arbitrarily set the size of $\mathcal{J}_c$ to 10\% of the overall number of network sites,i.e., we will assume the presence of $13$ anomalies in the considered network scenario. 
%-------------Correlazione tra 10 realizzazioni dei siti sotto performanti , meno importante?--------------------------
%Figure \ref{fig:Similarity_sites} shows the correlation between 10 different sets of under-performing sites, drawn according to the specified rule, considering the TM and the EM separately. The correlation maps shows that our system has very little bias with respect to the choice of under-performing sites. This is probably due to the fact that, even though we drive the choice of anomalies through $P_c^{\mathcal{J}}$, probabilities $p_c(j)$ are low and close to each other, as shown in Figure \ref{fig:pdf_anomaly} (the greatest values are in the order of 2\%). However, as it will be shown later, this will turn into higher robustness of the performance of the anomaly detection method with respect to the working conditions.
%\begin{figure}[H]
%    \centering
%    \includegraphics[scale=0.7]{pics/Pdf_anomaly.png}
%    \caption{Pdf over site ids, showing the probability for each site to be under-performing due to traffic congestion.}
%    \label{fig:pdf_anomaly}
%\end{figure}
%
%
%------------------------------------------------------------
% \subsection{User Profiler}\label{sec:UT}
%  %$\in$ $\mathcal{R}$
% The User Profiler (UP) simulates the subjective reactions of cellular users to their experience in the network. Let $s(i) \in \textbf{s}$ be a binary satisfaction label representing the reaction of user $i$, which equals $1$ if the user is \textit{dissatisfied} about his/her experience in the network, while it equals $0$ otherwise. Considering the set of under-performing sites $\mathcal{J}_u$ (which is an input to this block as shown in Figure \ref{fig:simframe}), the UP sets $s(i)=1$ for all users $i$ that satisfy the following condition:
% \begin{align}\label{eq:user_sat}
%    &\quad& \sum_{j \in \mathcal{J}_c} t\textsubscript{i,j} \geq u_i * \mathcal{H} &\quad&\forall{j} \in \mathcal{J}
% \end{align}
% where $\mathcal{H}$ is an arbitrary observation period. Therefore, $s(i)=1$ if the cumulative relative time spent by user $i$ in each visited under-performing site (if any) is greater than a user dependent time activation threshold, which is referred to as \textit{user tolerance} ($u_i \in [0,1]$). The rationale behind this rule is that if a user spends most of his/her time in an under-performing site (or equivalently in a group of them), then he/she will report a negative feedback to the operator. In other words, we assume that each user has a unique patience level (i.e., $u_i$) with respect to negative network experiences. Intuitively, the higher the tolerance of a user the more he/she will tolerate low service quality during his/her network activity. Considering that the population of users is heterogeneous, we decided to draw for each user $i$ the corresponding tolerance value from a Gaussian-distributed random variable $\mathcal{N}$ with mean $\mu$ and standard deviation $\sigma$, i.e., $u_i \sim \mathcal{N}(\mu, \sigma^2)$. Later in Section \ref{sec:sensan} we will discuss about the choice of their values.\par
% To conclude, considering that in general the satisfaction of a user regarding the cellular service depends also on non-network factors which relate to users personal attitudes and expectations~\cite{boz2019mobile}, the UP models such behaviours by setting $\psi$\% of the satisfaction labels $r(i)$ at random, regardless the user tolerance $u_i$. Thus, $\psi$ represents a hyper-parameter of the model that can be set by the operator to simulate different population types.
%~\cite{boz2019mobile} --> da aggiungere alla motivazione del rumore 15% sui voti
%We hypothesize that beyond a certain threshold (hereafter: the QoE saturation threshold), a significantly larger fraction of bad QoE events is related to non-network factors such as app quality, device performance, and user expectations, etc. These non-network features are more difficult to measure and capture and thus prediction performance decreases. Under this assumption, future mobile QoE studies will need to be multidisciplinary as these non-network features are related to many different academic domains, such as user experience, consumer psychology, and economics.

%\subsection{Survey Delivery}
%The most straightforward way that Telco operators have to measure their users' QoE is to directly ask them what is their satisfaction about the service received in a previous, recent period. 
%This is usually done by delivering a large quantity of satisfaction surveys, either via online messaging or through ad-hoc mobile applications. The success of a satisfaction survey campaign, which is typically expensive and cumbersome to undertake, can be measured in terms of the surveys \textit{Response Rate} ($RR$), i.e, the percentage of answers with respect to the overall number of delivered surveys. Clearly, the more the answers the better is the statistic representation of the customers population. However, due to the fact that usually cellular customers spend little time to answer satisfaction surveys, response rates are usually lower than $5\%$ \cite{pimpinella2019towards}. A possibility for the operators to augment this information is to i) learn how users reply to survey, correlating the received responses with objective information regarding users experience in the network (e.g. accessibility, traffic, etc. KPIs) and ii) build a model to predict unknown satisfaction feedbacks. Leveraging the matrix $\mathcal{T}$, the QEI works as it follows: 
% The Survey Delivery (SD) block is in charge of simulating the process of administration of satisfaction surveys from a cellular operator to its customers. The higher the \textit{response rate} ($\eta$) of a surveying campaign (i.e., the percentage of users answering the surveys with respect to the overall number of delivered surveys) the better is the statistic representation of the users population. We will consider two different surveys delivery strategies:
% \begin{itemize}
% 		\item Random Delivery (RD): with this policy, surveys are randomly delivered to the customers. This strategy is represented in Figure \ref{fig:random}, where user icons represent those who reply to the received survey while the base station icons represent the network sites. As one can note, in this unlucky example the operator has no information regarding the satisfaction of all those users visiting most of the anomalous sites (i.e. redish base stations), since few of them have answered the satisfaction survey. In other words, when such cases happen, the operator would have little chance to detect all the anomalies in the network.
% 		\item Optimized Delivery (OD): with this policy, the operator delivers surveys such to maximize the number of network sites \textit{covered} by the set of replying users. From now on, we will assume that a network site is covered if it has been visited at least by $n$ replying users, each one visiting the site for at least $l\%$ of the observation period. This scenario is depicted in Figure \ref{fig:optimum}, where replying users are distributed in the network such that the majority of the sites are covered. Intuitively, this lets the operator have a more clear understanding about network users satisfaction. Note that the greater the values of $n$ and $l$ the stricter the definition of network coverage, as either more or longer visiting users are needed to cover a network site. Both $n$ and $l$ represent system hyper-parameters that can be chosen a priori for modelling purposes.
% \end{itemize}
% \begin{figure}[t]
% \centering
% \subfigure[RD: low network coverage \newline scenario]{\label{fig:random}\includegraphics[width=0.38\textwidth]{pics/GTusersRandom.png}}
% \subfigure[OD: high network coverage \newline scenario]{\label{fig:optimum}\includegraphics[width=0.4\textwidth]{pics/GTusersOpt.png}}
% \caption{Strategies for the delivery of satisfaction surveys: a network coverage perspective. User icons refer to the users who replied to the received surveys, while blackish and redish base stations refer to regular and anomalous network sites respectively.}
% \label{fig:deliveries}
% \end{figure}
% From a simulative perspective, the SD block samples the set of users reactions $\mathbf{s}$ and returns a set of GT users feedbacks $\mathbf{s}\textsubscript{gt}$. 

\subsection{Under-Performing Sites Ranking and Detection}\label{sec:satprediction}
At this point, the detection system introduced in the previous Section (which corresponds to the core of the framework represented in Figure \ref{fig:simframe}) can be used to detect under-performing sites in the network. The system will leverage: i) the user-specific cell visit times information generated by the UMM; ii) the set of GT survey responses generated by the SD block and a pre-trained ML model $f(\cdot)$, to predict the satisfaction feedback of all those users who did not answer a survey. Note that the ML model is assumed to be already trained and detailing which learning features belong to $\mathbf{X}_\text{a}$ and $\mathbf{X}_\text{na}$ is outside the scope of this paper. For the sake of clarity, we underline that this block is blinded about the true location of the under-performing sites, i.e., it does not know which network site belongs to $\mathcal{J}_u$.%Finally, the system provides the operator with a ranked set $\hat{\mathcal{J}}_\text{u}$ of predicted under-performing sites, that is eventually compared with the set $\mathcal{J}_\text{u}$ to assess the detection performance.

%At this point, we can apply a method to detect under-performing sites in a cellular network. In this work, we will leverage: i) the set $\mathbf{s}\textsubscript{gt}$ of GT users feedbacks, ii) the vectors $\textbf{t}$(i) for each user $i$ in the visiting population and iii) the set of predicted feedbacks $\hat{\mathbf{s}}$ of those users not answering the received satisfaction survey. For the sake of clarity, we underline that this block is blinded about the true location of the under-performing sites, i.e., it does not know which network site belongs to $\mathcal{J}_u$.

For each network site in the network topology, the block computes a score $r_j$ according to the following procedure: 
\begin{enumerate}
	\item First, the set $\mathcal{V}_j$ of all the dissatisfied visitors of site $j$ is selected. Note that $\mathcal{V}_j$ contains all those users such that $t_{i,j}>0$ and the associated ground truth or predicted satisfaction is 0. We recall that a user visits multiple sites and its dissatisfaction may be due only to one of them. To cope with this, we tighten the time constraint as it follows:
	\begin{equation}
		t_{i,j} > \xi \sum_j t_{i,j}
	\end{equation}
where $\xi$ is a percentage that acts as an activation threshold for considering site $j$ as responsible to the experience of the $i$-th user. Further details about the choice of the value of $\xi$ will be given in Section \ref{sec:sensan}. 
	
\item Then, the site score is computed by summing all normalized user visit times above the threshold $\xi$, that is:
	\begin{equation}
    r_j = \sum_{i \in \mathcal{V}_j} \frac{t_{i,j}}{\sum_j t_{i,j}}.
	\end{equation}
%The rationale behind this way of scoring is that the longer the time spent by a dissatisfied visitor in site $j$ the more likely that site was responsible of user $i$ negative experience. In fact, the greater $r_j$ the higher the probability that site $j$ is under-performing as greater score values mean that many dissatisfied users have visited site $j$ for a relative time greater than the threshold $\xi$.
\end{enumerate}
Finally, network sites are ranked in descending order according to $r_j$ and the operator may use such an information to prioritise upgrading investments in the network. Here we assume that the operator has a budget for upgrading $k$ network sites. Feeding the value of $k$ into the detection system allows to output a set $\hat{\mathcal{J}}_\text{u}$, $|\hat{\mathcal{J}}_\text{u}| = k$, containing the first $k$ sites of the ranked list.

In the following Section we run the simulation framework in different scenarios and we compare the ranked set $\hat{\mathcal{J}}_\text{u}$ with the true set of under-perfoming cells $\mathcal{J}_\text{u}$ to assess the detection performance.






%Eventually, the block outputs a set $\hat{\mathcal{J}}_u$ of \textit{predicted} anomalies which contains the top $k$ ranked network sites. In this way, an operator can exploit the output of the block to prioritise upgrading investments in the network, thus finding an answer to question \ref{Q1} raised at the beginning of the Section. Note that in general the operator does not know in advance the exact number of under-performing or malfunctioning sites in the network, which makes the choice of the hyper-parameter $k\%$ not trivial. As an example, small values of $k\%$ can prevent the system to detect all the anomalies in the network. In the following Section we will discuss about the performance of the detection system with respect to different working scenarios.

%On the other hand, considering that in general economic resources are limited, large values of $k\%$ can confuse the operator about which site to prioritise for performing maintenance activities. 
%\begin{enumerate}
%\item First, it delivers satisfaction surveys to the whole users population. We will analyse two surveys delivery strategies: 
%\begin{itemize}
%		\item Random Delivery (RD): with this policy, surveys are randomly delivered to the customers. This strategy is represented in Figure \ref{fig:random}, where user icons represent those who reply to the received survey while the base station icons represent the network sites. As one can note, in this unlucky example the operator has no information regarding the QoE of all those users visiting most of the anomalous sites (i.e. redish base stations), since few of them have answered the satisfaction survey. In other words, when such cases happen, the operator would have little chance to detect all the anomalies in the network.
%		\item Optimized Delivery (OD): with this policy, the operator delivers surveys such to maximize the number of network sites \textit{covered} by the set of replying users. From now on, we will assume that a network site is covered if it has been visited at least by $n$ replying users, each one visiting the site for at least $l\%$ of the observation period. This scenario is depicted in Figure \ref{fig:optimum}, where replying users are distributed in the network such that the majority of the sites are covered. Intuitively, this lets the operator have a more clear understanding about the QoE of its customers in the network. Note that the greater the values of $n$ and $l$ the stricter the definition of network coverage, as either more or longer visiting users are needed to cover a network site. Both $n$ and $l$ represent system hyper-parameters that can be chosen a priori for modelling purposes.
%%In this work, we fix $k=20\%$ and $n=3$. 
%\end{itemize}
%	\item Secondly, regardless the delivery strategy, it returns a set $\mathcal{I}_{GT}$ of \textit{Ground Truth} users, corresponding to those users who replied the received survey. Note that $\mathcal{I}_{GT}$ $\subset$ $\mathcal{I}$, i.e., it is a subset of the whole users population. The size of $\mathcal{I}_{GT}$ depends on the response rate $RR$, which therefore represents a system hyper-parameter. At this point, we define $f_i$ as the survey response of user $i$, such that:
%	\begin{align*}
%	&\quad& f_i = r(i) &\quad&\forall{i} \in \mathcal{I}_{GT}
%	\end{align*}
%where $r(i)$ is the user's \textit{true} satisfaction label. Note that in the simulation framework such labels are generated by the UP, which in fact simulates users' responses to the surveys. 
%In fact, we assume that a ground truth user will provide the operator with the information of his/her true reaction to the experience in the network, which corresponds to the satisfaction label generated by the UPB.
%In other words, the ground truth users let the operator exactly know whether they had a positive or negative experience in the network.
%	\item Finally, it will predict the satisfaction feedbacks of all those users who have not replied to the received survey, such that:
%	\begin{align*}
%	&\quad& f_i = \hat{r}(i) &\quad&\forall{i} \notin \mathcal{I}_{GT}
%	\end{align*}
%	where $\hat{r}(i)$ is the \textit{predicted} satisfaction label of user $i$. Note that $\hat{r}(i)$ might be different than the true satisfaction label of user $i$. The case in which $\hat{r}(i) \neq r(i)$ happens when the QEI incurs in a \textit{prediction error}: we will later discuss upon the impact that prediction errors have into the anomaly detection process.
%\end{enumerate}
%To conclude, at the end of this process, the QEI outputs a set of feedbacks $\mathcal{F}$ which contains both the ground truth (i.e., $r(i)$) and the predicted ($\hat{r}(i)$) users satisfaction labels.
%As an example, network operators can increase the response rate introducing a reward system in the voting procedure, such that a user is rewarded (e.g. premium data plan access for limited time, etc.) if he/she answers the received survey (\cite{shah2015approval}). However, we recall that our aim is not just to collect information about users satisfaction of the experienced cellular service, but to exploit such information to perform anomaly detection in the network.
%\subsubsection{Anomaly Detector (AD)}\label{sec:anomalydetectionmethod}
%The AD implements a method to detect anomalies in a cellular network. Note that the AD is blinded about the location of the true anomalies, i.e., it does not know which network site belongs to $\mathcal{J}_c$.  
%To perform the detection task, the AD leverages the knowledge about i) users visits in the network (i.e., the mobility matrix $\mathcal{T}$) and ii) users feedbacks partially retrieved from a surveying campaign and partially predicted after the use of a classifier (i.e., the satisfaction labels $f(i) \in  \mathcal{F}$). \\
%For a given network site $j$ $\in$ $\mathcal{J}$, the AD works as it follows:
%\begin{enumerate}
%	\item First, it selects all the \textit{dissatisfied visitors} of site $j$, i.e., all those users $i$ such that $f(i)=0$ and that satisfy the following condition:
%	\begin{equation}
%		t_{i,j} > TTA*\mathcal{H}
%	\end{equation}
%	where TTA stands for \textit{Time Threshold for Anomaly} and is a hyper-parameter of the system. In particular, it represents a time activation threshold and defines the minimum percentage of time that a user has to spend in site $j$ in order to be considered its visitor. Further details about the choice of the value of TTA will be given in Section \ref{sec:sensan}. 
%	\item Secondly, it assigns to site $j$ a \textit{score}, namely $R_{0}(j)$, defined as it follows:
%	\begin{align}
%    &R_{0}(j) = \sum_{i \in \mathcal{V}_d(j)} \frac{t_{i,j}}{T_{i}}
%	\end{align}
%	where $\mathcal{V}_d(j)$ is the set of dissatisfied visitors of site $j$. The rationale behind this way of scoring is that the longer the time spent by a dissatisfied visitor in site $j$ the more likely that site has been responsible of user $i$ negative feedback. In fact, the greater $R_{0}(j)$ the higher the probability that site $j$ is anomalous as greater score values mean that many dissatisfied users have visited site $j$ for a relative time greater than the threshold $TTA$.
%\end{enumerate}
%\begin{figure}[t]
%\centering
%    \includegraphics[scale=0.7]{pics/AnomDet.png}
%    \caption{Schema representing the flow of operations needed to detect under-performing sites.}
%    \label{fig:3.9}
%\end{figure}
%

%\textbf{* * * * * * *  * * *Experiments Details 2* * * * * * * * * * * * *}
%-------------------Confronto diverse Ranking Rule --> Non ne parlerei-----------------------------------------
%% RANKING SCORES
%In this work, two Ranking Rules are considered and compared, namely $R_{0}$ and $R_{1}$:
%\begin{align}
%    &R_{0}(j) = \sum_{\substack{i \in \mathcal{S}_{uns},\\ t_{i,j} > TTA*TH}} \frac{t_{i,j}}{T_{i}} \\ 
%    &R_{1}(j) = \dfrac{\sum\limits_{\substack{i \in \mathcal{S}_{uns},\\ t_{i,j}>TTA*TH}} t_{i,j} \cdot \frac{t_{i,j}}{T_{i}}}{T_{j}} 
%\end{align}
%The former Ranking Rule (3.6) is very simple: it only takes into account the percentage of time spent by dissatisfied users in site j. Using this rule, we are able to weight individual scores according to the amount of time they spent in j: users that spent a considerable amount of time in that site are considered as more reliable, thus they contribute more to the site end score.
%The latter Ranking Rule (3.7) contains all the above ingredients mentioned above. This choice is driven by the fact that our purpose is to understand the differences that lie in the choice of the Ranking Rule.
%\par In order to compare the performance in the utilization of each Ranking Rule, we have to briefly introduce a performance metric, which will be discussed later on in detail: the AUC score. When considering a binary classification algorithm, the performance depends on the way in which it classifies each data point: based on the number of correctly classified points and misclassified ones, several metrics can be computed. One of the most popular performance metric is the so called Receiver Operating Characteristic (ROC) curve: it is a curve where the true positive rate (a.k.a. TPR), i.e. the portion of positive correctly classified samples with respect to the total number of positive samples, is plotted as a function of the false positive rate (a.k.a. FPR), i.e. the portion of negatives that were incorrectly classified as positive with respect to the total number of negative samples. The AUC score is simply the Area Under the Curve of the ROC curve: intuitively, the higher this value, the higher the performance of the classifier, reaching the value 1 when the classifier correctly predicts every new data point.
%% Diagramm
%In Figure \ref{fig:Diagram3} a diagram summarizing the system described before is shown. We evaluated the AUC values as a function of the TTA parameter for the ranking scores $R_{0}(j)$ and $R_{1}(j)$ respectively and showed the result in Figure \ref{fig:3.10}.
%\begin{figure}[H]
%    \centering
%    \includegraphics[scale=0.65]{pics/ComparisonScores_2.png}
%    \caption{AUC versus TTA for the two considered ranking rules.}
%    \label{fig:3.10}
%\end{figure}
%As we can see, we can conclude that:
%\begin{itemize}
%    \item the performance of both ranking scores is quite high, with values in the range 92\%-98\%: thus, the choice of the ranking rule used for detection is not binding; 
%    \item the performance trends are quite flat, hence the performance are robust with respect to the choice of the value of \textit{TTA}. This is important, as in principle it is not know what is the minimum amount of time that a user has to spend in a network site to consider that site relevant for the assessment of the quality of his/her overall experience in the network.
%\end{itemize}
%Due to these conclusions, for the following steps of this thesis work, we decide to choose $R_{0}(j)$ as reference ranking rule, with a fixed $TTA$ value of 0.2.
%\par
%-----------------------------------------




